Diagrammatic Polyhedral Algebra

We extend the theory of Interacting Hopf algebras with an order primitive, and give a sound and complete axiomatisation of the prop of polyhedral cones. Next, we axiomatise an affine extension and prove soundness and completeness for the prop of polyhedra.

==> Garbage.tex <==
%
%
% PETRI NETS STUFFS
%
%




%\begin{example}\label{ex:Petri-nets}
%Consider the Petri net displayed below with the usual graphical notation: circles represent places, and squares transitions.
%\begin{center}
%\begin{turn}{-90}
%\begin{tikzpicture}[node distance=.5cm,>=stealth',bend angle=45,auto]
%    \node [pl] (p1)                                    {};
%    \node [pl] (p2) [left=.5cm of p1]                      {};
%    \node [pl] (p3)  [right=.5cm of p1] {};
%    \node [pl] (p4)  [above=1.2cm of p1] {};
%
%    \node [transition] (t1) [above left=.5cm and .25cm of p1] {}
%      edge [pre]                  (p1)
%      edge [post]                (p2)
%      edge [post]                           (p4);
%    \node [transition] (t1) [above right=.5cm and .25cm of p1] {}
%      edge [pre]                  (p1)
%      edge [post]                (p3)
%      edge [post]                           (p4);
%    \node [transition] (t3) [below left=.5cm and .25cm of p1] {}
%      edge [post]                  (p1)
%      edge [pre]                (p2);
%    \node [transition] (t4) [below right=.5cm and .25cm of p1] {}
%      edge [post]                  (p1)
%      edge [pre]                (p3);
%\end{tikzpicture}
%\end{turn}
%\end{center}
%By fixing a left-to-right and top-to-bottom ordering, $\pre{-}$ and $\post{-}$ of the leftmost net are represented by the matrices $\begin{pmatrix} 3 &1 \\0&0\end{pmatrix}$ and $\begin{pmatrix} 0&0 \\ 6&2\end{pmatrix}$ and for the rightmost by $\begin{pmatrix} 1 \\0\end{pmatrix}$ and $\begin{pmatrix} 0 \\ 2\end{pmatrix}$.
%\end{example}

Petri nets are combinatorial objects, usually studied monolithically rather than compositionally.
%To overcome this issue, there have been many proposals---\cite{Mazurkiewicz,Baldanetal,Sobocinski2010,Bruni,Baez,Reisig} amongst others---for calculi of \emph{open nets}, roughly speaking, composable nets equipped with some sort of interface. %We postpone a more detailed comparison to these works in Section \ref{}.
%
%Hereafter,
We introduce a syntax $\CircP$ that \textit{(i)} compiles to CSFGs in a straightforward way and \textit{(ii)} whose \emph{closed} diagrams (arrows in $\CircP[0,0]$) capture precisely the behaviour of continuous Petri nets. Moreover, arbitrary diagrams (arrows in $j\to k$) are open nets, reminiscent to those in~\cite{Bruni2013}.

%The essential point is that Petri net places are  \emph{asynchronous buffers}, with behaviour that of the following stateful resource calculus diagram:
%\PS{Instead of repeating it here, it would be better to refer to an earlier sighting}
%\[\tikzfig{buffer}\]
%Intuitively, a token stored in $\register$ can non-deterministically leave on  the right, or be fed back into $\register$ through the loop. Exploiting the isomorphism of Theorem \ref{thm:processes}, the interpretation of the asynchronous buffer in $\mathsf{St}(\AddRel)$ % is canonical and
%matches the operational semantics of Definition~\ref{def:Petri-net} exactly.



%We now introduce the calculus of Petri nets and we show that this can be encoded into the stateful variant of the resource calculus. We will then motivate the name, by showing that Petri nets can be naturally encoded into the Petri calculus.
%
%\medskip

The syntax is~\eqref{eq:syntax} extended with one extra generator $\place: (1,1)$ intuitively representing a Petri net place. Formally, its operational behaviour is given by the following rule.
\begin{equation}\label{eq:ruleplace}
\derivationRule{i,o,m\in\posreals, \quad o\leq m}{(\place,m)  \dtrans{i}{o} (\place,m-o+i)}{}
\end{equation}
We use $\semantics{c}$ to denote the resulting relation, defined analogously to~\eqref{eq:operationalStateful}.
Like in Section~\ref{sec:calculus}, we consider diagrams obtained from the syntax to be morphisms of a prop $\CircP$. It is useful to observe that $\CircP$ is the same as the coproduct $\Circ + \Pl$ in $\PROP$, where $\Pl$ is the prop whose arrows are string diagrams on the signature $\{\place\}$.
The relevant equational theory is $\Petri \df \RC + \Pl$, the quotient of $\CircP$ by $=_{\RC}$ (Figure \ref{fig:resource-calc-axioms}).
%We call $\Pl$ the prop  generated by $\place$, with no equations, $\CircP \df \Circ + \Pl$ the prop for the syntax, and


%In Section \ref{sec:encode-Petri} we demonstrate how Petri nets can be considered as closed diagrams of $\Petri$ and establish the formal correspondence of their behaviours. Then, in Section \ref{sec:behaviour-Petri}, we show that $\Petri$ can be embedded into the resource calculus, interpreting the place as an asynchronous buffer.



\subsection{Encoding nets into $\Petri$}
\label{sec:encode-Petri}

%Before rigorously defining
We illustrate the role of $\Petri$ with the aid of an example.
\begin{example}
%   The circuits in $\RC$ corresponding to the matrices for the nets in Example \ref{ex:Petri-nets}  are displayed below
%$$INSERT \quad FIGURE \quad EXAMPLE 1,2,3,4 $$
The diagrams of $\Petri[0,0]$ corresponding to the net of Example \ref{ex:Petri-nets} is:
%\[\tikzfig{ex-Petri-diagram}\]
More generally, a place with multiple inputs and outputs is depicted as
%\[\tikzfig{generic-place}\]
using \Wmult and \Wcomult, while transitions are represented with the help of \Bmult and \Bcomult.
\end{example}

Any ordinary Petri net $\mathcal{P}$ can be encoded as a diagram $d_{\mathcal{P}}$ in $\Petri[0,0]$.
By choosing an ordering on places and transitions, the functions $\pre{-},\post{-}\from T\to \N^P$ can be regarded as $\N$-matrices of type $|T| \to |P|$. Such matrices can be seen as special cases of additive relations (\emph{cf.} Theorem~\ref{thm:mat}, Section \ref{sec:mat}): let $s$ and $t$ be the diagrams in $\RC$ corresponding to $\pre{-}$, $\post{-}$ respectively.
We let %then take the diagram
 $d_\mathcal{P}$ be % to be %\[d_{\mathcal{P}} \df \Tr{s^{-1}\poi t}_{|P|}\]
$$\tikzfig{encoding-Petri-a}$$
That this assignement is well-defined is proven in Appendix~\ref{app:petrinets}.
%
It is easy to show that $\mathcal{P}$ and $d_\mathcal{P}$ have the same operational behaviour.

%\begin{lemma}\label{lemma:trcaeoperational}
%Let $d\in \RC[n+p,m+p]$ and ${\mathbf{a}}, {\mathbf{b}}$ be a vector in $\N^p$.
%\[(\mathbf{a}}, {\mathbf{w_1}}, {{\mathbf{b}}, {\mathbf{w_2}})\in \sem{d}  \text{ iff } (\mathbf{a'}}, {\mathbf{w_1'}}, {{\mathbf{b'}}, {\mathbf{w_2'}})\in \sem{TR_p(d)}\] for all $w_1 \in \N^n$, $w_2\in \N^m$ and ${\mathbf{a'}},{\mathbf{b'}} \in \N^p$ such that ${\mathbf{a'}}\leq {\mathbf{a}}$ and ${\mathbf{b}}={\mathbf{a}}-{\mathbf{a'}}+{\mathbf{b'}}$.
%\end{lemma}
%\begin{proof}
%TO BE DONE, I GUESS IT IS BY INDUCTION ON $\Petri$
%\end{proof}



\begin{proposition}\label{prop:encPT1}
Given a Petri net $\mathcal{P}$, we have $\sem{\mathcal{P}}\sim \sem{d_\mathcal{P}}$.
\end{proposition}
\begin{proof}
In Appendix~\ref{app:petrinets}.
\end{proof}
Similarly, for every diagram $d \in \Petri[0,0]$, one can construct a Petri net $\mathcal{P}_d$ with the following recipe: by Lemma \ref{lem:trace-form}, $d$ can be written in trace canonical form, namely there exists a diagram $c\in\RC[p,p]$ such that \eqref{eq:tracecanform} holds. The diagram $c$ denotes an additive relation $\isoRC(c)\subseteq \N^p\times \N^p$ that, by Proposition \ref{thm:minimal-rep}, has a Hilbert basis. This basis can be represented as matrix $A\colon t \to p+p$ for some $t\in \N$ representing the dimension of the basis. The matrix $A$ can be decomposed into two matrices $A_1,A_2\colon t\to p$ such that $A=\bigl( \begin{smallmatrix} A_1 \\ A_2\end{smallmatrix} \bigr)$. We define  $\mathcal{P}_d \df (p,t,A_2,A_1)$, that is $p$ and $t$ (seen as ordinal sets) are the set of places and transitions, $A_1$ and $A_2$ play the role of $\pre{-}$ and $\post{-}$.




Again, it is easy to prove that the operational behaviour is preserved.
\begin{proposition}\label{prop:encPT2}
For all $d\in \Petri[0,0]$, $\sem{d} \sim \sem{\mathcal{P}_d }$
\end{proposition}
\begin{proof}
In Appendix \ref{app:petrinets}.
\end{proof}
%\begin{example}\label{exPN2} We now take as circuit $c$, the one in \eqref{} and we apply the transformation on it. Since it is already in trace canonical form, it is easy to see that the corresponding circuit $d$ is the one in \eqref{}. Observe that the additive relation $I(d)$ is the one generated by the leftmost matrix below that has as Hilbert basis the set on the right.
%$$\begin{pmatrix} 3 &1 \\0&0\\0&0\\6&2\end{pmatrix} \quad \quad \quad \left\{\begin{pmatrix} 1 \\0\\0\\2\end{pmatrix}\right\}$$
%Therefore, the matrix $A_1$ and $A_2$ are $\begin{pmatrix} 1 \\0\end{pmatrix}$ and $\begin{pmatrix} 0\\2\end{pmatrix}$: the net corresponding to $c$ is isomorphic to the one in \eqref{}. \end{example}


%Examples \ref{ex:irredundant} and \ref{exPN2} show that by encoding first the net in \eqref{} into a circuit and then encoding the corresponding circuit into a net, one obtains the net in \eqref{} which is not isomorphic to \eqref{}. Still the two nets have the same operational behaviour.

By virtue of Propositions \ref{prop:encPT1} and \ref{prop:encPT2} together, Petri nets and diagrams in $\Petri[0,0]$ are in one-to-one correspondence modulo semantic equivalence.


%\subsection{Embedding $\Petri$ in $\RCS$}
\subsection{Classifying stateful extensions}
\label{sec:behaviour-Petri}
%The calculus of Petri nets can be encoded into the stateful resource calculus in a rather straightforward way.
%In the Introduction we
Recall that diagram $c_2$~\eqref{eq:introEx} in the introduction behaves like a place of a Petri net. We now use it to embed $\Petri$ in $\RCS$. The prop morphism $\encodingPetri{-}\colon \CircP \to \CircS$ takes:
\begin{equation}
  \label{eq:place-buffer}
\encodingPetri{\place}\df \quad %\tikzfig{buffer}
\end{equation}
and acts as the identity for the constants of $\Circ$.
Following the discussion in Section \ref{sub:expressiveness}, it is immediate that ${\encodingPetri{\place}}$ is exactly the behaviour defined by~\eqref{eq:ruleplace}, that is
\begin{equation}\label{eq:opcorrespondence}\sem{\encodingPetri{\place}} = \{(m,i,m',o) \mid o\leq m \text{ and }m'=m-o+i \} =  \sem{\place}\end{equation}
A simple induction allows us to extend the correspondence $\eqref{eq:opcorrespondence}$ to all diagrams in $\CircP$ .
\begin{proposition}\label{prop:presNet}
Given arbitrary $c\in \CircP$, $\sem{\encodingPetri{c}}\sim \sem{c}$.
\end{proposition}
The above proposition together with Corollary \ref{cor:CompletenessRCS} guarantee the following.
\begin{corollary}\label{cor:presNet}
For all diagrams $c,d$ of $\CircP$, $\sem{c} \sim \sem{d}$ if and only if $\encodingPetri{c} =_\RC \encodingPetri{d}$.
\end{corollary}

We have shown that the stateful resources calculus is at least as expressive as $\Petri$ (and thus Petri nets). We shall now show that $\Petri$ is \emph{strictly less expressive} than the stateful resource calculus, in the sense that not all transition systems definable by $\RCS$ can be expressed by diagrams in $\Petri$. Intuitively, this is because the register of the resource calculus is \emph{synchronous} whereas the place of Petri nets is \emph{asynchronous}, namely it can always perform a transition that does not change its internal state. This property holds for all diagrams of the Petri calculus: % as stated by the following.
%
%As we have shown above, the asynchronous buffer can be encoded from a synchronous register, using nondeterminism and a feedback operation. We now show that we cannot encode the register of the resource calculus taking the Petri net place as primitive.
%
%%The following theorem shows that all the transition systems that Petri nets can express have a run that does not change the internal state.
%\begin{proposition}\label{prop:Petri-constant-state}
%  For every diagram $d$ in $\CircP$, there exists some additive relation $R$ such that
%\[\mathsf{id}_s\otimes R\subseteq \sem{c}_p\]
%\end{proposition}
%\begin{proof}
%If $s=0$, this is immediate. Otherwise, we can show it by induction, since
%\[\left\llbracket\tikzfig{identity-zero}\right\rrbracket\quad \subseteq \quad \left\llbracket\tikzfig{place-lts}\right\rrbracket = \left\llbracket\place\right\rrbracket_p\]
%\end{proof}
%\begin{corollary}
%$\register$ is not in the image of~$\mathcal{E}\colon \mathsf{Petri}\to\mathsf{Rc}_m$.
%\end{corollary}
%\begin{proof}
%It is straightforward to see that $\sem{\sym}$ does not contain a relation that can be factorized as in Proposition \ref{prop:Petri-constant-state}.
%\end{proof}
%Hence,
%\begin{proposition}
%$\Petri$ is strictly less expressive than $\RCS$
%\end{proposition}
Recall that we define the semantics of a diagram $d$ of $\CircP$ as the relation:
\begin{equation}\label{eq:operationalStateful}
\sem{d} \df  \{(\bm{s}_1,\bm{a},\bm{s}_2,\bm{b}) \mid (d,\bm{s}_1) \dtrans{\bm{a}}{\bm{b}}(d,\bm{s}_2)\} \subseteq \N^R \times \N^k\times \N^R \times \N^l  \text{.}
\end{equation}
\begin{proposition}\label{prop:Petri-constant-state}
Let $d$ be in $\CircP$. Then %$({\mathbf{a}}, {\mathbf{0}},{\mathbf{a}}, {\mathbf{0}})\in \sem{d}$
$({\mathbf{a}}, {\mathbf{0}},{\mathbf{a}}, {\mathbf{0}})\in \sem{d}$
for all ${\mathbf{a}}$.
\end{proposition}
\begin{proof}
By induction. %on $\CircP$.
The only case of interest is $\place$, and $(a, 0, a, 0)\in \sem{\place}$ by \eqref{eq:ruleplace}.
\end{proof}
Given that $(a, 0, a, 0)\not \in \sem{\register}$ unless $a = 0$, we immediately obtain:
\begin{corollary}\label{cor:petriinexpressive}
For all diagrams $d$ in $\CircP$, $\sem{d}\not \sim \sem{\register}$. \qed
\end{corollary}
%Hence,
%\begin{proposition}
%$\Petri$ is strictly less expressive than $\RCS$
%\end{proposition}




%\begin{theorem}
%For all diagrams $d$ in $\Petri$, $\isoRCS(\encodingPetri{d}) =\semPetri{d}$.
%\end{theorem}
%\begin{proof}
%TO BE DONE
%\end{proof}

%\medskip

%\noindent It easy to check that $\sem{\place} \sim \sem{\encodingPetri{\place}}$ and, by induction, that $\sem{d} \sim \sem{\encodingPetri{d}}$ for all $d\in \CircP$. Corollary \ref{cor:CompletenessRCS} entails then the following result.
%\begin{theorem}
%For all diagrams $c,d$ in $\CircP$, $\sem{c} \sim \sem{d}$ iff $\encodingPetri{c} =_{\RC}\encodingPetri{d}$.
%\end{theorem}
%\begin{proof}
%Let $[-]_{\RC} \colon \Circ \to \RC$ be the functor mapping each circuit in its equivalence class.
%We first prove the commutation of the following diagram.
%
%\[
%\xymatrix{
%\Circ + \Pl  \ar[dd]_{id_{\Circ}+\encodingPetri{-}} \ar[r]^{[-]_{\RC}+id_{\Pl}} & \RC+\Pl \ar[d]^{\langle Z,P\rangle}\\
%& \stFul{\RC}\\
%\Circ + X  \ar[r]_{[-]_{\RC}+id_{X}} & \RC+X \ar[u]_{\langle Z,R\rangle}
%}
%\]
%
%\end{proof}

%Observe that $\Petri=\RC+\Pl$ where $\Pl$ is the prop freely generated by $\place$. By Theorem \ref{thm:processes}, $\Petri$ is isomorphic to $\mathsf{St}(\AddRel)$, but the functor $\isoRCS$ witnessing the isomorphism assigns to $\place$ the same operational behaviour of $\register$.


The expressivity result strengthens the claim that $\register$ is a ``more canonical'' way than $\place$ to introduce state to $\AddRel$. Indeed, in Section~\ref{sec:axstate} we have seen that $\RCS$ is isomorphic to $\mathsf{St}(\AddRel)$. Now, because of Corollary \ref{cor:petriinexpressive}, it cannot be the case that $\Petri$ is also isomorphic to $\mathsf{St}(\RC)$.

Moreover, we can use the example of $\place$ to show in a more precise sense how the resource calculus plays the role of a yardstick, guiding the space of design choices for stateful extensions of additive relations. Once we know that the behaviour $\sem{\place}$ of $\place$ is an arrow of $\mathsf{St}(\AddRel)$, the encoding $\encodingPetri{\place}$ of $\place$ in the resource calculus is completely determined. Using the isomorphisms $\langle Z,R \rangle \colon \RCS \to \mathsf{St}(\RC)$ and $\mathsf{St}(\isoRC) \colon \mathsf{St}(\RC)\to \mathsf{St}(\AddRel)$ from Section \ref{sec:stateful} we have:
\[  \mathsf{St}(\isoRC)^{-1}(\sem{\place})  =
  \left(1,\tikzfig{place-lts}\right)
  \]
and
\begin{align*}
  \langle Z,R\rangle^{-1}\left(1,\tikzfig{place-lts}\right)
  \ &= \  \langle Z,R\rangle^{-1}\left(1,\tikzfig{state-buffer-2} \right)
  \\[2ex]
  &= \  \langle Z,R\rangle^{-1} \left(1,\tikzfig{state-buffer-1} \right)
  \\[2ex]
  &= \ \langle Z,R\rangle^{-1}  \left(1, \tikzfig{state-buffer} \right)
  \\[2ex]
  &= \ \tikzfig{buffer} \ = \ \encodingPetri{\place}
\end{align*}

This computation evaluates $\sem{\place}$ both to a stateful diagram from $\RCS$ (the conclusion)  and a pair in $\mathsf{St}(\Circ)$ of a state and a stateless diagram (first equality). Notice the difference with the interpretation $(1,\sym)$ that the isomorphism $\isoRCS$ gives to $\register$ in $\mathsf{St}(\Circ)$.

Intriguingly, the same kind of analysis can be performed to other stateful extensions of $\AddRel$. One example from the literature is the \emph{banking semantics}~\cite{Bruni2011,Bruni2013} of Petri nets, which defines behaviour differently:

%its operational behaviour is given by the following rule.
\[
\derivationRule{m+i=m'+o}{(
\tikzfig{place-b},m)  \dtrans{i}{o} (
\tikzfig{place-b},m')}{}.
\]
Applying the same computations to $\sem{
\tikzfig{place-b}}$ defined in terms of the banking rule, one obtains following representations in $\mathsf{St}(\Circ)$ and in $\RCS$:
\[  \mathsf{St}(\isoRC)(\sem{\tikzfig{place-b}}) = \left(1,\tikzfig{banking-lts}\right) \text{ and } \langle Z,R\rangle^{-1}\mathsf{St}(\isoRC)(\sem{\tikzfig{place-b}})= \bigl( \tikzfig{buffer-banking} \bigr) \]

For each notion of state, Figure~\ref{places} displays the associated diagrams in $\mathsf{St}(\RC)$ and $\RCS$. %Our argument for
The canonicity of $\sem{\register}$ is witnessed by the fact that, for any possible operational semantics $\sem{\place}$ in $\mathsf{St}(\AddRel)$ that one may want to give to $\place$, one obtains diagrams in $\mathsf{St}(\RC)$ and $\RCS$.
\begin{figure}[t]
\begin{tabular}{c|cc}
& $\mathsf{St}(\RC)$ & $\RCS$\\
\hline\\
$\sem{\register}$ & $(1, \sym)$ & $\register$ \\
\hline\\
$\sem{\place}$ & $\left(1,\tikzfig{place-lts}\right) $ & $\left(\tikzfig{buffer}\right)$\\ \hline \\
$\sem{
\tikzfig{place-b}}$ & $ \left(1,\tikzfig{banking-lts}\right)$ & $\bigl( \tikzfig{buffer-banking} \bigr)$
\end{tabular}\caption{For each of the semantics on the left, the central and the right columns report the corresponding arrows in $\mathsf{St}(\RC)$ and $\RCS$.}\label{places}
\end{figure}



%
%given  by
%the same expression as equation (\ref{eq:place-buffer}), but now the RHS is quotiented by the equations of $\RC$. To obtain the transition systems associated with diagrams of $\Petri \df \RC+\Pl$, we pair $\mathsf{Buff}$ with $Z$ and compose it with $\langle Z,R\rangle$ and $\stFul{I}$ from Section \ref{sec:process}, to define a functor  $\semPetri \colon \Petri \to \mathsf{St}(\AddRel)$:
%\[\semPetri \df \Petri \xrightarrow{\langle Z,\mathsf{Buff}\rangle} \RCS \xrightarrow{\langle Z,R\rangle} \stFul{\RC} \xrightarrow{\stFul{I}}  \stFul{\AddRel}\]
%From this, we derive the behaviour of the place purely diagrammatically.
%\begin{proposition}\label{prop:place-lts}
%\[\langle Z,R\rangle\langle Z,\mathsf{Buff}\rangle(\place)=\left(1,\tikzfig{place-lts}\right)\]
%\end{proposition}
%\begin{proof}
%As no confusion arises, in the following we omit the first component of the above pair.
%%we omit from the proof the $1$ in the pair of the statement above.
%  \begin{multline*}
%    \langle Z,R\rangle\langle Z,\mathsf{Buff}\rangle(\place) \ = \  \langle Z,R\rangle\left(\tikzfig{buffer}\right)
%     \ =\ \tikzfig{state-buffer}\\
%      = \ \tikzfig{state-buffer-1} \ = \  \tikzfig{state-buffer-2}  \ = \ \tikzfig{place-lts}
%  \end{multline*}
%\end{proof}
%From this last diagram of $\stFul{\AddRel}$, it is straightforward to derive the behaviour of the place and verify that it corresponds to expected operational semantics.
%\begin{corollary}
%  \[\semPetri(\place) = \left\{ \big(\bigl( \begin{smallmatrix}m\\i\end{smallmatrix} \big), \big( \begin{smallmatrix}m-o+i\\o \end{smallmatrix} \big)\big) \mid m,o,i\in \N \text{ and } o\leq m \right\}\]
%\end{corollary}

%
%
%It is worth noting that, by Theorem \ref{thm:processes}, $\Petri$ is isomorphic to $\mathsf{St}(\AddRel)$, but $\semPetri$ is \emph{not} an isomorphism since we do not map the place to $\sym$. In fact, $\Petri$ is strictly less expressive than the stateful resource calculus: not all transition systems in $\stFul{\AddRel}$ can be expressed by diagrams in the image of $\semPetri$. Intuitively, this is because the register of the resource calculus is \emph{synchronous} whereas the place buffer of Petri nets is \emph{asynchronous}, namely it can always perform a transition that does not change its internal state. This property holds for all diagrams of the Petri calculus as stated by the following result.
%
%As we have shown above, the asynchronous buffer can be encoded from a synchronous register, using nondeterminism and a feedback operation. We now show that we cannot encode the register of the resource calculus taking the Petri net place as primitive.
%
%%The following theorem shows that all the transition systems that Petri nets can express have a run that does not change the internal state.
%\begin{proposition}\label{prop:Petri-constant-state}
%  For every diagram $d$ in $\CircP$, there exists some additive relation $R$ such that
%\[\mathsf{id}_s\otimes R\subseteq \sem{c}_p\]
%\end{proposition}
%\begin{proof}
%If $s=0$, this is immediate. Otherwise, we can show it by induction, since
%\[\left\llbracket\tikzfig{identity-zero}\right\rrbracket\quad \subseteq \quad \left\llbracket\tikzfig{place-lts}\right\rrbracket = \left\llbracket\place\right\rrbracket_p\]
%\end{proof}
%\begin{corollary}
%$\register$ is not in the image of~$\mathcal{E}\colon \mathsf{Petri}\to\mathsf{Rc}_m$.
%\end{corollary}
%\begin{proof}
%It is straightforward to see that $\sem{\sym}$ does not contain a relation that can be factorized as in Proposition \ref{prop:Petri-constant-state}.
%\end{proof}
%Hence,
%\begin{proposition}
%$\Petri$ is strictly less expressive than $\RCS$
%\end{proposition}

%\begin{proposition}\label{prop:Petri-constant-state}
%Let $d$ be a diagram in $\CircP$. Then $({\mathbf{a}}, {\mathbf{0}},{\mathbf{a}}, {\mathbf{0}})\in \sem{d}$ for all ${\mathbf{a}}$.
%\end{proposition}
%\begin{proof}
%By induction on $\CircP$. The only non-trivial base case is that of the place, for which one can check that $({\mathbf{a}}, {\mathbf{0}},{\mathbf{a}}, {\mathbf{0}})\in \sem{\place}$.
%\end{proof}
%\begin{corollary}
%For all diagrams $d$ in $\CircP$, $\sem{d}\not \sim \sem{\register}$.
%\end{corollary}
%\begin{proof}
%It is enough to observe that $({\mathbf{a}}, {\mathbf{0}},{\mathbf{a}}, {\mathbf{0}})\not \in \sem{\register}$.
%\end{proof}
%%Hence,
%%\begin{proposition}
%%$\Petri$ is strictly less expressive than $\RCS$
%%\end{proposition}

%
%\begin{remark}\label{canonicityOfRegister}
%There real difference between $\Petri$ and $\RCS$ is in their operational semantics: they both contain generators of the same type that satisfy the same equations. The distinguishing feature comes from the interpretations of $\register$ as a synchronous register and $\place$ as an asynchronous buffer. The isomorphism of Theorem \ref{thm:processes} shows that the interpretation of the register into $\stFul{\AddRel}$ is the most general, placing the fewest constraints on the behaviour of processes constructed from it and the other basic components of the resource calculus. But, if our interpretation of the place was guided by the operational semantics of Petri nets, there are as many interpretations of the additional $1\to 1$ generator as there are functors $F\colon \Pl \to \stFul{\RC}$. For instance $F(\place)=\left(1,\Wmult \poi \Wcomult\right)$ would give us  the so-called \emph{banking semantics} from \cite{} defined by
%\[
%\derivationRule{m+i=m'+o}{\place^m  \dtrans{i}{o} \place^{m'}}{}.
%\]
%%Moreover, by virtue of such result, for any possible semantics defined via some $F\colon \Pl \to \stFul{\RC}$, one can always find an encoding of $\Pl$ into $\RCS$ defined as
%%\[\xymatrix{\Pl \ar[r]^F & \stFul{\RC} \ar[r]^{<Z,R>^{-1}} &\RCS }\]
%%Indeed, by using the definition of $<Z,R>^{-1}$ that we gave in the proof of Theorem \ref{}, the reader can readily check that $<Z,R>^{-1}(P(\place)) =_{\RC} \encodingPetri{\place}$.
%\end{remark}

%\begin{remark}\label{thm:linear-buffer-fail}
%It is worth highlighting the crucial role of our departure from linear to additive relations. Observe that if in the operational semantics in Section \ref{} we would have considered vectors over sets with negative values (like $\mathbb{Z}$ or $\mathbb{R}$), then the aynchronous buffer that we used to encode places would have been equal to the total relation:
%\[ \left\llbracket \tikzfig{buffer}\right\rrbracket \quad = \quad \left\llbracket \tikzfig{proof-linear-buffer-13}\right\rrbracket \]
%Indeed, the possibility of storing negative values in the register allows to have transitions with arbitrary numbers on the left and on the right ports.
%\end{remark}


%\subsection{Encoding open Petri nets}
%{\bf FB: Decide what to do with this...}
%In this section we study the connection with open Petri nets as defined in \cite{}.

%
% OLD VERSION BOUNDED
%
%\subsection{Bounded Petri nets}
%So far, we have tested the expressiveness of the stateful resource calculus with P/T Petri nets. Using a similar approach, we now show that its affine variants, $\RCSA$, can express \emph{bounded} Petri nets.
%
%In a bounded Petri nets each place has a  maximal number of tokens that it may contain. Hereafter we restrict to $1$-bounded Petri nets, also known as C/E nets, where \emph{all} places can contain at most one token. The extension to arbitrary bounded nets is straightforward.
%
%Using the same arguments of Section \ref{sec:behaviour-Petri}, one can show that $1$-bounded nets can be embedded into the calculus of bounded Petri nets, $\textsf{BPetri}$, having the same syntax as $\CircP$ but with the following semantics for the 1-bounded place $\tikzfig{place-1}$.
%\begin{equation}\label{eq:rulebplace}
%%\derivationRule{A}{B}{}
%\derivationRule{o\leq m\leq 1 \quad m-o+i \leq 1}{(\tikzfig{place-1},m)  \dtrans{i}{o} (\tikzfig{place-1},m-o+i)}{}
%\end{equation}
%%Note that this is a ``reasonable stateful extension'' in the sense of the previous section, if working with the affine resource calculus.
%% $\PolyRel$.
%Indeed, it is immediate to see that the above rule just restricts \eqref{eq:ruleplace} with the additional constraint that the actual number of token stored in the place ($m$) and the next one ($m-o+i$) are smaller than $1$. This constraint can be easily expressed using the affine resource calculus, as we already seen for the stateless connectors in Section \ref{sec:statelessconn}, where we defined $\idSmallerOne$.  The prop morphism relevant here, $\encodingPetri{-}\colon \CircP \to \CircSA$,
%% behaves like the identity for the constants of $\Circ$, while it
%maps $\place$ to the following:
%%\PS{Can we make this diagram less crammed?}
%\begin{equation*}
%  \label{eq:place-buffer}
%\encodingPetri{\place}\df \quad \tikzfig{bounded-buffer}
%\end{equation*}
%It is straightforward to see that the analogous of Proposition \ref{prop:presNet} and Corollary \ref{cor:presNet} holds.


==> conc.tex <==
\section{Conclusions and Future Work}
This work extends the theory of Interacting Hopf Algebra with $\greq$ and $\One$, resulting in a complete theory for axiomatic reasoning over polyhedra. On the one hand, this is a powerful diagrammatic calculus for convex algebra, which we demonstrate by proving several well-known theorems; on the other, it provides the basis for a calculus that extends signal flow graphs and is an intriguing model of concurrency. Indeed, using the theory in~\cite[\S 4]{BHPSZ-popl19}, the addition of a single generator, $\circuitXT$, leads to the calculus of stateful polyhedral processes which is expressive enough to encode continuous Petri nets.

Several papers~\cite{Meseguer1990,DBLP:conf/apn/BestDH92,DBLP:conf/concur/NielsenPS95,DBLP:conf/apn/Kindler97,DBLP:journals/mscs/BaldanCEH05,bruni2011connector,Bruni2013,DBLP:journals/mscs/BaezM20,DBLP:journals/corr/abs-2101-04238}
have studied the problem of providing Petri nets with a compositional semantics, but to the best of our knowledge, only one work~\cite{Master_2020} provides a calculus for continuous Petri nets. More precisely,~\cite{Master_2020} introduces a compositional semantics for $Q$-nets for an arbitrary Lawvere theory $Q$, thus encompassing continuous Petri nets. The approach is rather different from ours: $Q$-nets are regarded as $Q$-structured spans and a free construction provides the process semantics;  moreover, axiomatizations are not studied.

It is worth to remark that the semantics equivalence that we characterise, $\sim$, is just some form of $\alpha$ equivalence hiding the names of registers. This is definitively too intensional to be considered an observational semantics, like bisimilarity or trace equivalence. Thanks to the abstract theory presented in~\cite{DBLP:conf/concur/BonchiPSZ19}, bisimilarity in our calculus is a congruence and we know that the same holds also for trace equivalence. However providing a complete axiomatization for this kind of semantics is a challenging task that we leave as future work.

==> figures/poly/aihaxioms.tex <==
\begin{equation*}
    \tikzfig{one-copy} \myeq{dup} \tikzfig{one2} \qquad 
    \tikzfig{one-delete} \myeq{del} \tikzfig{empty-diag} \qquad 
    \tikzfig{one-false} \myeq{\emptyset} \tikzfig{one-false-disconnect} \qquad 
\end{equation*}

==> poly.tex <==
\section{The theory of Polyhedra}\label{sec:poly}
In this section we extend $\IHP{\mathsf k}$ in order to capture polyhedra. 
Recall that a polyhedra over an ordered field $\field$ is a set $P\subseteq \field^n$ such that $P = \{ x \in \field^n \mid Ax +b \geq 0 \}$ for some matrix $A$ and some vector $b$. Observe that the emptyset $\emptyset$ is a polyhedron, but not a polyhedral cone. For our development, it is pivotal the notion of homogenization. The \emph{homogenization} of the polyhedra $P$ is the polyhedral cone $P^H = \{ (x, y) \in \field^{n+1} \mid Ax + by \geq 0, y \geq 0 \}$.

\begin{lemma}\label{th:polyinc}
Let $P_1, P_2 \subseteq \field^n$ be two non-empty polyhedra. Then,
%\[ P_1 = \{ x \in \field^n \mid Ax \leq b \} \;\;\;
%P_2 = \{ x \in \field^n \mid Cx \leq d \}\]
%and their \textit{homogenisations}
%\[ P_1^H = \{ \begin{pmatrix} x \\ y\end{pmatrix} \in \field^{n+1} \mid \begin{pmatrix} A & -b \\ %0 & -1\end{pmatrix}\begin{pmatrix} x \\ y\end{pmatrix} \leq 0 \} \] \[
%P_2^H = \{ \begin{pmatrix} x \\ y\end{pmatrix} \in \field^{n+1} \mid \begin{pmatrix} C & -d \\ 0 & -1\end{pmatrix}\begin{pmatrix} x \\ y\end{pmatrix} \leq 0 \}\]
%It holds that 
$P_1 \subseteq P_2$ iff $P_1^H \subseteq P_2^H$.
\end{lemma}

\begin{definition} \label{def:p} $\propCat{P}_{\mathsf k}$ is the sub-PROP of $\RelX{\mathsf k}$ where arrows $n \rightarrow m$ are polyhedra $\{ (x,y) \in \field^n \times \field^m \mid A\begin{pmatrix*} x \\ y \end{pmatrix*} + b \geq 0 \}$ for some matrix $A$ and vector $b$. Identities, permutations, composition and monoidal product are defined as in $\RelX{\mathsf k}$.
\end{definition}

In order to denote polyhedra, our language needs to be able to express constant vectors like $b$ above. This can be done by adding to our signature the generator
\begin{equation}\label{eq:perp}
\One
\end{equation}
having semantics $\dsem{\One}=\{(\nullvec, 1)\}$. We call $\ACDP$ the PROP freely generated by \eqref{eq:SFcalculusSyntax1}, \eqref{eq:SFcalculusSyntax2}, \eqref{eq:>} and \eqref{eq:perp}.
Now, every arrow $P\colon n \to m$ of $\propCat{P}_{\mathsf k}$, that is $P=\{ (x,y) \in \field^n \times \field^m \mid A\begin{pmatrix*} x \\ y \end{pmatrix*} + b \geq 0 \}$ is denoted by the following diagram in $\ACDP$, where \input{figures/polyc/pnf-def1} and \input{figures/poly/b-diag} are diagrams in $\FC$.
\begin{equation}\label{eq:polynf}
\input{figures/poly/Nf1-general}
\end{equation}
%\marginpar{Nelláltra sezione era $p$. Cerchiamo di essere consistenti...}
\begin{proposition}[Expressivity]\label{th:ihpiso}
    For each arrow $P \colon n \rightarrow m$ in $\propCat{P}_{\mathsf k}$ there exists a circuit $c \colon n \rightarrow m$ in $\ACDP$, such that $P = \dsemp{c}$. Viceversa, for each circuit $c \colon n \rightarrow m$ of $\ACDP$ there exists an arrow $P \colon n \rightarrow m$ of $\propCat{P}_{\mathsf k}$, such that $\dsemp{c} = P$. 
\end{proposition}



%Figure \ref{fig:aihpaxioms} ill

%We call $\AIHP{\mathsf k}$ the PROP freely generated by the above signature and the axioms in Figure \ref{fig:aihpaxioms}. 
The three axioms on left of Figure \ref{fig:aihpaxioms} describe the interaction of $\One$ with the generators in \eqref{eq:SFcalculusSyntax1}. These were introduced in \cite{BonchiPSZ19} and proved complete w.r.t. affine relations (i.e., sets of solutions of systems of the shape $Ax +b = 0$). %Particularly interesting is the axiom $\emptyset$: the empty polyhedron $\emptyset = \{(\nullvec, 1)\} ; \{(0, \nullvec)\} =\dsem{\onefalse}$ behaves as a logical false, since for any relation $R$ in $\RelX{\field}$, $R \oplus \emptyset = \emptyset = \emptyset \oplus R$. 
%
To obtain a complete axiomatisation for polyhedra, we only need to one extra axiom $AP1$ stating just that $1\geq 0$. We call $\AIHP{\mathsf k}$ the PROP freely generated by \eqref{eq:SFcalculusSyntax1}, \eqref{eq:SFcalculusSyntax2}, \eqref{eq:>}, \eqref{eq:perp} and the axioms Figures \ref{fig:ih}, \ref{fig:axiom:ihp} and \ref{fig:aihpaxioms}.

%\begin{figure}
%    \input{figures/poly/aihaxioms}
%    \caption{Axioms of $\AIH{\field}$}
%    \label{fig:aihaxioms}
%\end{figure}



\begin{figure}
%    \input{figures/poly/aihaxioms}
    \input{figures/poly/aihp-axioms}
    \caption{Axioms of $\AIHP{\field}$}
    \label{fig:aihpaxioms}
\end{figure}
With these axioms, any circuit in $\ACDP$ is equivalent to one in the form of \eqref{eq:polynf}. This can be easily proved by mean of the first normal form theorem for $\CDP$ (Theorem \ref{th:polynf}) and the following lemma.

\begin{lemma}\label{lm:nf2}
For any  $c \colon n \rightarrow m$ of $\ACDP$, there exists $c' \colon n+1 \rightarrow m$ of $\CDP$ such that 
\input{figures/poly/nf2-def}
\end{lemma}

\begin{theorem}\label{th:nf}
For all $c$ of $\ACDP$, there exist $d$ in the form of \eqref{th:polynf} such that $c \myeq{\AIHP{}} d$.
%\input{figures/poly/nf1-def}
\end{theorem}
%\marginpar{Ater the corrections are made, please put this proof it in the Appendix}

%\marginpar{Talk here about Homozenitation in the standard regular way abd then describe wjat it means axiomatically}

%\begin{definition}\label{def:homog}
%    Let $P = \{ x \in \field^n \mid Ax + b \geq 0\}$ be a polyhedron. Its homogenisation is the polyhedral cone
%    \[ P^H = \{ (x, y) \in \field^{n+1} \mid Ax + by \geq 0, y \geq 0 \} \]
%\end{definition}

%\begin{definition}\label{def:homogd}
%    Let $c \colon n \rightarrow 0$ be an arrow of $\AIHP{\mathsf k}$ representing the polyhedron %${\{ x \in \field^n \mid Ax + b \geq 0\}}$
%
%\begin{center}
%\input{figures/poly/polyhedron}
%\end{center}
%Its homogenisation is represented by the arrow $c^H \colon n+1 \rightarrow 0$ of $\IHP{\mathsf k}$ obtained by replacing the $\One$ in $c$ with a diagram representing the constraint~$\geq 0$
%\begin{center}
%    \input{figures/poly/hpolyhedron}
%\end{center}
%\end{definition}
Using the above theorem and homogenization (Lemma~\ref{th:polyinc}), we can reduce completeness for non-empty polyhedra to completeness of polyhedral cones.
\begin{theorem}\label{th:compl}
Let $c, d \colon n \rightarrow m$ be circuit of $\ACDP$ denoting two \textit{non-empty} polyhedra. If
$\dsem{c} \subseteq \dsem{d}$, then $c \stackrel{\AIHP{}}{\subseteq} d$.
\end{theorem}

To prove completeness for empty polyhedra, we need few additional lemmas, illustrated in Appendix \ref{app:poly} for lack of space.

\begin{theorem}\label{th:compl2}
For all circuits $c$ in $\ACDP$, if $\dsem{c}=\emptyset$ then $c \myeq{\AIHP{}} \tikzfig{one-false-disconnect}$ %\marginpar{Insert diagram here}
%representing an \textit{empty} polyhedron, then the following holds
%\begin{equation*}
%\input{figures/poly/compl2-def}
%\end{equation*}
\end{theorem}

\begin{corollary}
[Completeness]\label{co:compl}
For all circuits $c$ in $\ACDP$, if 
$\dsem{c} \subseteq \dsem{d}$ then $c \stackrel{\AIHP{\field}}{\subseteq} d$.
\end{corollary}

\begin{corollary}
$\AIHP{\field} \cong \propCat{P}_{\mathsf k}$
\end{corollary}




==> polyc.tex <==
\section{The Theory of Polyhedral cones}\label{sec:polyc}
We now extend $\IH{\mathsf k}$ so as to express polyhedral cones over an \emph{ordered} field $\field$. Recall that a field $\field$ with a total order $\leq$, is said to be ordered if the following properties hold: for any $i,j,k \in \field$: (a) if $i \leq j$, then $i + k \leq j + k$; (b) if $0 \leq i$ and $0 \leq j$, then $0 \leq ij$.
A \emph{polyhedral cone} over $\field^n$ is a set $C\subseteq \field^n$ such that $C=\{ x \in \mathsf{k}^{n} \mid A x \geq 0 \}$ for some matrix $A$. The Weyl-Minkowski theorem provides an alternative characterization of polyhedral cones in terms of finitely generated (f.g.) cones: an aribitrary subset $S\subseteq \mathsf{k}^{n}$ is \emph{a f.g.\ cone} if $S=\mathsf{cone}(V)$ for some finite set of vectors $V=\{v_1, \ldots , v_m\}$, where $\mathsf{cone}(V) = \{ k_1 v_1 + \ldots + k_m v_m \mid k_i \in \mathsf{k}, \,k_i\geq 0\}$.

\begin{definition} \label{def:pc} $\propCat{PC}_{\mathsf k}$ is the sub-PROP of $\RelX{\mathsf k}$ where arrows $n \to m$ are polyhedral cones $\{ (x,y) \in \mathsf{k}^{n}\times \mathsf{k}^{m} \mid A\begin{pmatrix*} x \\ y \end{pmatrix*} \geq 0 \}$ for some matrix $A$. Identities, permutations, composition and monoidal product are as in $\RelX{\mathsf k}$.
\end{definition}
Showing that $\propCat{PC}_{\mathsf k}$ is well-defined---e.g., that the composition of two polyhedral cones is a polyhedral cone---requires some well-known results, which we provide in Appendix \ref{app:standardproperties}.

\medskip

To obtain an appriopriate diagrammatic syntax,
we extend the signature in \eqref{eq:SFcalculusSyntax1}, \eqref{eq:SFcalculusSyntax2} with the following generator:
\begin{equation}\label{eq:>}
\greq
\end{equation}
and call the PROP freely generated by this extended signature $\CDP$.
The semantic map $\dsempO \colon \CDP \rightarrow \RelX{\mathsf k}$ behaves exactly as $\dsemO$ for the generators in \eqref{eq:SFcalculusSyntax1} and \eqref{eq:SFcalculusSyntax2}, whereas on $\greq$ it is defined as hinted by our syntax: $\dsemp{\greq}=\{\; (x, y) \mid x, y \in \mathsf{k},\, x \geq y \;\}$.
%\begin{equation}
%\greq \longmapsto \{ (x, y) \mid x, y \in \mathsf{k}, x \geq y \}
%\end{equation}

It easy to see that an arbitrary arrow $C\colon n \to m$ of $\propCat{PC}_{\mathsf k}$, i.e., $C= \{ (x,y) \in \mathsf{k}^{n}\times \mathsf{k}^{m} \mid A\begin{pmatrix*} x \\ y \end{pmatrix*} \geq 0 \}$ for some matrix $A$, can be expressed by the following diagram in $\CDP$.
\begin{equation}\label{eq:polyhedralcnf}
\input{figures/poly/Ihpgeneric}
\end{equation}
Above, \input{figures/polyc/pnf-def1} is a diagram of $\FC$ denoting the matrix $A$ (see Example \ref{ex:matrix}).
%The proof of the following result, reported in Appendix \ref{sec:polyc}, consists in just checking that the semantics of \eqref{eq:polyhedralcnf} coincides with the $C$.
%
\begin{proposition}[Expressivity] \label{th:ihpiso}
    For each arrow $C \colon n \rightarrow m$ in $\propCat{PC}_{\mathsf k}$ there exists an circuit $c \colon n \rightarrow m$ of $\CDP$, such that $C = \dsemp{c}$. Viceversa,
    for each circuit $c \colon n \rightarrow m$ of $\CDP$ there exists an arrow $p \colon n \rightarrow m$ of $\propCat{PC}_{\mathsf k}$, such that $\dsemp{c} = p$.

%    Meaning that $\dsempO$ factors via a functor $\dsemO' \colon \CDP \rightarrow \propCat{PC}_{\mathsf k}$ and the obvious embedding $I$ of $\propCat{PC}_{\mathsf k}$ into $\RelX{\mathsf k}$, i.e. such that the following diagram commutes
%    \[% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVANwIYBsCuMkgA6hAxgJYBOJACrggDQgAOEcZALmRGEsgAz0+AXQC+9dNjwFiJDO2AAlGFhEB9YMQC2cgBZwAZgAIA1iJCMWbTt14BGQaPEhMufIiKk5wagGE1Gwm12PSNTc2ZWDi4eFHtbUSFGGCgAc3heCVdpQig4GE0AeQBycKwMACNlakjrGJAKMhSddnD9CghNJAEQdggkACYxTKl3Ylz8pnxGMsqsaqtogiwYfRbGNo6uxl6kWyHnSTcPAEkIdgxSiqqaxfcGprWejDIsAh0ICGNsR43OxH7tn1EHtREA
%    \begin{tikzcd}
%    \CDP \arrow[rd, "\dsemO'"'] \arrow[r, "\dsempO"] & \RelX{\mathsf k}                          % \\
%                                                          & \propCat{PC}_{\mathsf k} \arrow[u, "I"', hook']
%    \end{tikzcd}\]
\end{proposition}
%The proof, reported in full details in Appendix \ref{sec:polyc}, is by induction on $\CDP$: one has just to check the property for the generators, since the inductive cases are trivial by functoriality of $\dsempO$.

\medskip

The above proposition  provides an answer to the problem of expressivity: $\CDP$ denotes all and only the polyhedral cones. We can now face the problem of axiomatisation. % semantic equivalence and inclusion.

We denote by $\IHP{\mathsf k}$ the PROP freely generated by the theory consisting of the above signature (namely, \eqref{eq:SFcalculusSyntax1}, \eqref{eq:SFcalculusSyntax2} and \eqref{eq:>}, the axioms of $\IH{\mathsf k}$ and the axioms in Figure \ref{fig:axiom:ihp}: the axioms on the first two rows describe the interactions of $\greq$ with the generators in \eqref{eq:SFcalculusSyntax1}. The axioms in the third row assert that $\geq$ is reflexive, transitive and antisymmetric: BLA BLA. The only axiom in the last row is somehow more peculiar: the right-to-left inclusion states that for all $k_1,k_2,l_1,l_2 \in \field$, if $k_i\geq l_j$ for all $i,j=1,2$, then there exists some $u$ such that $k_i \geq u \geq l_i$. The left-to-right inclusion is redundant.

The diagram $\leqd$ appearing in the axioms is defined as $\greqop$, by means of the compact closed structure (see Example~\ref{ex:cc}).

\begin{figure}
\input{figures/polyc/ihp-axioms}
\caption{Axioms of $\IHP{\field}$}\label{fig:axiom:ihp}
\end{figure}

Routine computations confirm that all the axioms are sound. Proving completeness requires to illustrate axiomatic proofs of several standard results.

\begin{proposition}[Fourier-Motzkin elimination]\label{prop:FMElimitation}
For each arrow $A \colon n \rightarrow m$ of $\FC$, there exits an arrow $B \colon n-1 \rightarrow l$ of $\FC$ such that
\input{figures/polyc/fm1}
\end{proposition}
The proof, in Appendix \ref{app:FMelimination}, consists in a string diagrammatic derivation mimicking the Fourier-Motzkin elimination, an algorithm for eliminating variables from a system of linear inequalities (i.e. projecting a polyhedral cone).

The next step consists in illustrating a normal form theorem. A circuit $c \colon n \rightarrow m$ of $\CDP$ is said to be in \emph{polyhedral normal form} if there is an arrow \input{figures/polyc/pnf-def1} of $\FC$, such that $c=\eqref{eq:polyhedralcnf}$.
\begin{theorem}
    \label{th:polynf}
    For each arrow $c \colon n \rightarrow m$ of $\CDP$, there is another arrow $d \colon n \rightarrow m$ of $\CDP$ in polyhedral normal form such that $c \myeq{\IHP{}} d$.
\end{theorem}
The proof goes by induction on the structure of $\CDP$.
The most challenging case is the sequential composition which makes use of the Fourier-Moztkin elimination. All details can be found in Appendix \ref{app:polynf}.

Diagrams in $\CDP$ enjoys a second normal form: an arrow $c \colon n \rightarrow m$ of $\CDP$ is said to be in \textit{finitely generated normal form} if there is an arrow \input{figures/polyc/fnf-def1} of $\FCop$, such that
\[ c =  \input{figures/polyc/fnf-def2} \]
It is easy to check that $\dsemp{c}$ is the \textit{finitely generated cone} $\{ (x,y) \in \mathsf{k}^{n}\times \mathsf{k}^{m} \mid \begin{pmatrix*} x \\ y \end{pmatrix*} = Vv, v \geq 0 \}$.
To prove the existence of this normal form, we need to introduce the polar operator, an important construction in convex analysis which, in our approach, enjoy a simple inductive definition.%which benefits of a involutive property on closed convex cones, and specifically on polyhedral cones.
%Given that the arrows of $\CDP$ faithfully represent polyhedral cones, we define the operator directly on them.

\begin{definition}
    The \textit{polar} operator $\cdot^{\circ} \colon \CDP \rightarrow \CDP$ is the functor inductively defined as:
\[
\begin{array}{ccccc}
\Bcomult \ \longmapsto \ \Wcomult
&
\Bcounit \ \longmapsto \ \Wcounit
&
\tscalar{k} \ \longmapsto \ \tcoscalar{k}
&
\Wmult \ \longmapsto \Bmult
&
\Wunit \ \longmapsto \ \Bunit
\\
\Bmult \ \longmapsto \Wmult
&
\Bunit \ \longmapsto \ \Wunit
&
\tcoscalar{k} \ \longmapsto \ \tscalar{k}
&
\Wcomult \ \longmapsto \ \Bcomult
&
\Wcounit \ \longmapsto \ \Bcounit
\end{array}
\]

\[
\begin{array}{ccc}
\input{figures/polyc/polarpolar-geq} & (c \scolon d)^{\circ} = c^\circ \scolon d^\circ  & (c \oplus d)^{\circ} = c^\circ \oplus d^\circ
\end{array}
\]
\end{definition}

\begin{proposition} \label{th:polarpolar}
%\marginpar{Alessandro fai attenzione qui... Metti le prove corrispondenti in appendice, nel modo corretto...}
For all arrows $c,d \colon n \rightarrow m$ in $\CDP$, it holds that
\begin{enumerate}
    \item if $c \stackrel{\IHP{}}{\subseteq} d$ then $(d)^\circ \stackrel{\IHP{}}{\subseteq} (c)^\circ$;
    \item $(c^\circ)^\circ \myeq{\IHP{}} c$;
    \item if $c$ is an arrow of $\FC$, then $c^\circ$ is an arrow of $\FCop$.
\end{enumerate}
\end{proposition}

\begin{proposition}
    \label{th:polarfingen}
    For each arrow $c \colon n \rightarrow m$ of $\CDP$ in polyhedral normal form there is an arrow $d \colon n \rightarrow m$ of $\CDP$ in finitely generated normal form, such that $(c)^\circ \myeq{\IHP{}} d$.
\end{proposition}
\begin{proof}
    \input{figures/polyc/polarfingen-proof}
\end{proof}

%\marginpar{Alessandro, puoi accorciare il diagramma in lnea della prova in modo che tutto rientri nltima linea?}
\begin{theorem}[Weyl-Minkowski]
    \label{co:fingennf}
    For each arrow $c \colon n \rightarrow m$ of $\CDP$, there is an arrow $d \colon n \rightarrow m$ of $\CDP$ in finitely generated normal form such that $c \myeq{\IHP{}} d$.
\end{theorem}
\begin{proof}
    %Let $c^\circ$ be the polar cone of $c$.
    By Theorem \ref{th:polynf} there exists an arrow $p \colon n \rightarrow m$ of $\CDP$ in polyhedral normal form, such that $c^\circ \myeq{\IHP{}} p$. By Proposition \ref{th:polarpolar}.1 $p^\circ \myeq{\IHP{}} (c^\circ)^\circ$ and by Proposition \ref{th:polarpolar}.2 $ (c^\circ)^\circ \myeq{\IHP{}} c$, thus $p^\circ \myeq{\IHP{}} c$. Since $p$ is in polyhedral normal form, by Proposition \ref{th:polarfingen}, there exists a circuit $d$ in finitely generated normal form such that $d \myeq{\IHP{}} p^\circ \myeq{\IHP{}} c$.
\end{proof}
It is worth to remark that neither the polyhedral nor the finitely generated normal form are unique: different matrices may give rise to the same cone. However, with the finitely generated normal form, proving completeness requires only a few more lemmas, which for the sake of space, we report in Appendix \ref{app:completenessproofs}.

\begin{theorem}
    \label{th:compl2}
    For all circuits $c, d \in \CDP$, if $\dsemp{c} \subseteq \dsemp{d}$ then $c \mysubeq{\IHP{}} d$.
\end{theorem}
By the above theorem and Proposition \ref{th:ihpiso} follows that
\begin{corollary}
$\IHP{\mathsf k} \cong \propCat{PC}_{\mathsf k}$
\end{corollary}


%\begin{theorem}[Completeness]
%    \label{th:compl4}
%    For all circuits $c, d \in \CDP$, if $\dsemp{c} = \dsemp{d}$ then $c \myeq{\IHP{}} d$.
%\end{theorem}
%\begin{proof}
%    Trivially follows from Theorem \ref{th:compl2}.
%\end{proof}

